Classical and Quantum Features of the Mixmaster Singularity

This review article is devoted to analyze the main properties characterizing the cosmological singularity associated to the homogeneous and inhomogeneous Mixmaster model. After the introduction of the main tools required to treat the cosmological issue, we review in details the main results got along the last forty years on the Mixmaster topic. We firstly assess the classical picture of the homogeneous chaotic cosmologies and, after a presentation of the canonical method for the quantization, we develop the quantum Mixmaster behavior. Finally, we extend both the classical and quantum features to the fully inhomogeneous case. Our survey analyzes the fundamental framework of the Mixmaster picture and completes it by accounting for recent and peculiar outstanding results.

==> authors.tex <==
\author{GIOVANNI MONTANI
% \footnote{
% Typeset names in 8 pt roman, uppercase. Use the footnote to indicate the
% present or permanent address of the author.}
}

\address{ICRA, International Center for Relativistic 
	Astrophysics\\
	ENEA C.R. Frascati, Dipartimento F.P.N., 
	%via E. Fermi 45 - 00044, 
	Frascati, Roma, Italy\\
	 Dipartimento di Fisica 
		Universit\'a ``La Sapienza'', P.le a. Moro 5, 00185 Roma, Italy\\
	ICRANet, International Relativistic Astrophysics Network, Pescara, Italy\\
% University Department, University Name, Address\\
% City, State ZIP/Zone,
% Country\footnote{State completely without abbreviations, the
% affiliation and mailing address, including country. Typeset in 8 pt
% italic.}\\
	montani@icra.it}

\author{MARCO VALERIO BATTISTI}

\address{ICRA, International Center for Relativistic 
	Astrophysics\\
 	Dipartimento di Fisica 
	Universit\'a ``La Sapienza'', P.le a. Moro 5, 00185 Roma, Italy\\
% Group, Laboratory, Address\\
% City, State ZIP/Zone, Country\\
	battisti@icra.it}


\author{RICCARDO BENINI}

\address{ICRA, International Center for Relativistic 
	Astrophysics\\
 	Dipartimento di Fisica 
	Universit\'a ``La Sapienza'', P.le a. Moro 5, 00185 Roma, Italy\\
% Group, Laboratory, Address\\
% City, State ZIP/Zone, Country\\
	riccardo.benini@icra.it}


\author{GIOVANNI IMPONENTE}

\address{Museo Storico della Fisica e Centro Studi e Ricerche ``E. Fermi'', Roma, Italy\\
	Dipartimento di Fisica 
	Universit\'a ``La Sapienza'', P.le a. Moro 5, 00185 Roma, Italy\\
% Group, Laboratory, Address\\
% City, State ZIP/Zone, Country\\
	giovanni.imponente@cern.ch}



